A Unifying Perspective for Safety of Stochastic Systems: From Barrier Functions to Finite Abstractions

Providing safety guarantees for stochastic dynamical systems is a central problem in various fields, including control theory, machine learning, and robotics. Existing methods either employ Stochastic Barrier Functions (SBFs) or rely on numerical approaches based on finite abstractions. SBFs, analogous to Lyapunov functions, are used to establish (probabilistic) set invariance, whereas abstraction-based approaches approximate the stochastic system with a finite model to compute safety probability bounds. This paper presents a unifying perspective on these seemingly different approaches. Specifically, we show that both methods can be interpreted as approximations of a stochastic dynamic programming problem. This perspective allows us to formally establish the correctness of both techniques, characterize their convergence and optimality properties, and analyze their respective assumptions, advantages, and limitations. Our analysis reveals that, unlike SBFs-based methods, abstraction-based approaches can provide asymptotically optimal safety certificates, albeit at the cost of increased computational effort.

==> Input/Preliminary.tex <==
An interval Markov decision process (\imdp) is a generalization of a Markov decision process, where the probability of transition between each state-action pair lies within  intervals~\cite{givan2000bounded}. As we will see in this paper, having intervals to model transition probabilities allows one to efficiently represent uncertainties in the system dynamics.  
\begin{definition}[Interval MDP] \label{def:imdp}
    An \textit{interval Markov decision process} (IMDP) is a tuple $\I = (\Qimdp,\Aimdp,\Plow,\Pup)$ where
    \begin{itemize}
    	\setlength\itemsep{1mm}
    	\item $\Qimdp$ is a finite set of states,
    	\item $\Aimdp$ is a set of actions, where $\Aimdp(\qimdp)$ is the set of available actions at state $\qimdp\in \Qimdp$,
        \item $\Plow: \Qimdp \times \Aimdp \times \Qimdp \to [0,1]$ is a function, where $\Plow(\qimdp,\aimdp,\qimdpprime)$ defines the lower bound of the transition probability from state $\qimdp\in \Qimdp$ to state $\qimdpprime\in \Qimdp$ under action $\aimdp \in \Aimdp(\qimdp)$,
        \item $\Pup: \Qimdp \times \Aimdp \times \Qimdp \to [0,1]$ is a function, where $\Pup(\qimdp,\aimdp,\qimdpprime)$ defines the upper bound of the transition probability from state $\qimdp$ to state $\qimdpprime$ under action $\aimdp \in \Aimdp(\qimdp)$.
    \end{itemize}
    If $|A|=1$, then $\I$ is also called Interval Markov Chain (IMC).
\end{definition}
For all $\qimdp,\qimdpprime \in \Qimdp$ and $\aimdp \in \Aimdp(\qimdp)$, it holds that $\Plow(\qimdp,\aimdp,\qimdpprime) \leq \Pup(\qimdp,\aimdp,\qimdpprime)$ and
$
    \sum_{\qimdpprime \in \Qimdp} \Plow(\qimdp,\aimdp,\qimdpprime) \leq 1 \leq \sum_{\qimdpprime \in \Qimdp} \Pup(\qimdp,\aimdp,\qimdpprime).
$ That is, $\Plow$ and $\Pup$ represent valid lower and upper bounds of the transition probabilities.

Let $\distribution(\Qimdp)$ denote the set of probability distributions over $\Qimdp$.  
Given $\qimdp \in \Qimdp$ and $\aimdp \in \Aimdp(\qimdp)$, we call $\feasibleDist{\qimdp}{\aimdp} \in \probDist(\Qimdp)$ a \textit{feasible distribution} over states reachable from $\qimdp$ under $\aimdp$ if the transition probabilities respect the intervals defined for each possible successor state $\qimdpprime$, i.e., $\Plow(\qimdp,\aimdp,\qimdpprime)\leq\feasibleDist{\qimdp}{\aimdp}(\qimdpprime)\leq\Pup(\qimdp,\aimdp,\qimdpprime)$. 
We denote the set of all feasible distributions for state $\qimdp$ and action $\aimdp$ by $\FeasibleDist{\qimdp}{\aimdp}$.  
A path $\pathimdp$ of an \imdp is a sequence of state-action pairs $\pathimdp = \qimdp_0 \xrightarrow{\aimdp_0} \qimdp_1 \xrightarrow{\aimdp_1} \qimdp_2 \xrightarrow{\aimdp_2}  \ldots$ 
such that $\aimdp_i \in \Aimdp(\qimdp_i)$ and $\Pup(\qimdp_i, \aimdp_i, \allowbreak{\qimdp_{i+1}}) > 0$ 
for all $i \in \naturals$.
We denote the last state of finite paths by 
$\Pathimdpfin$. 
Actions taken by the \imdp are determined by a choice of strategy $\str$ which is defined below.

\begin{definition}[Strategy]
\label{def:strategy}
    A strategy $\str$ of an \imdp  $\, \I$ is
    a function $\str: 
    \Pathimdpfin 
    \to \Aimdp$ 
    that maps a finite path
    $\pathimdp$ of $\I$ onto an 
    action in $\Aimdp$. The set of all strategies is denoted by $\Str$.
\end{definition}

Once an action is chosen according to a strategy, a feasible distribution needs to be chosen from $\FeasibleDist{\qimdp}{\aimdp}$ to enable a transition to the next state.  
This task is performed by adversary function $\adv$ as
defined below. 
\begin{definition}[Adversary]
\label{def:adversary}
    Given an \imdp $\,\I$, an adversary is a function $\adv: \Pathimdpfin \times \Aimdp \rightarrow \probDist(\Qimdp)$ that, for each  finite path $\pathimdpfin \in \Pathimdpfin$ and action $\aimdp \in \Aimdp(\last(\pathimdpfin))$, chooses a feasible distribution $\feasibleDist{\qimdp}{\aimdp} \in \FeasibleDist{\last(\pathimdpfin)}{\aimdp}$. 
    The set of all adversaries is denoted by $\Adv$.
\end{definition}
Once an adversary is selected, then $\I$ reduces to an MDP. Similarly,  once a strategy and an adversary are selected, $\I$ results in a standard Markov chain.  Consequently, the key step in performing analysis with IMDPs is in synthesizing a pair (strategy, adversary). In Section \ref{sec:IMDPAbstraction} we will illustrate how in the case of probabilistic safety such a pair can be efficiently synthesized via linear programming. 
%Hence, given a strategy and an adversary, a probability measure can be defined on the paths of the $\imdp$ via the probability of paths on the resulting Markov chain~\cite{lahijanian2015formal}.

%In the next section, we show that by appropriate construction of an $\imdp$ abstraction for Process~\eqref{eq:system} through careful consideration of the transition kernel (Eq.~$\eqref{eq:transition-kernel}$) 
%and the regression error (Eq.~\eqref{eq:proberror}), the probability measures calculated from verifying the \imdp against a PCTL formula capture the true probability of Process~\eqref{eq:system} satisfying the formula.


